Study on Human-Variability-Respecting Optimal Control Affecting Human Interaction Experience

Broad application of human-machine interaction (HMI) demands advanced and human-centered control designs for the machine's automation. Human natural motor action shows stochastic behavior, which has so far not been respected in HMI control designs. Using a previously presented novel human-variability-respecting optimal controller we present a study design which allows the investigation of respecting human natural variability and its effect on human interaction experience. Our approach is tested in simulation based on an identified real human subject and presents a promising approach to be used for a larger subject study.

==> 1_tex/img/HRVC_system.tex <==

 \definecolor{shadecolor}{rgb}{0.92,0.92,0.92}

\tikzstyle{block} = [rectangle, draw, text width=2cm, text centered, minimum height=1.5cm]
 \tikzstyle{box} = [rectangle, draw, fill=shadecolor, text width=9em, text centered, rounded corners, minimum height=4em]
\tikzstyle{noise} = [rectangle, draw, text width=1.5cm, text centered, minimum height=0.8cm]
\tikzstyle{noiseS} = [rectangle, draw, text width=1cm, text centered, minimum height=0.8cm]
\tikzstyle{plus} = [circle, draw, text width=0.1cm, text centered]
 \tikzstyle{frame} = [rectangle, dashed, draw, text width=9em, text centered, minimum height=4em]


\tikzstyle{line} = [draw, -latex']

\usetikzlibrary{arrows}
\begin{tikzpicture}
 
 %system
\node[block, fill=shadecolor, text width=5cm, text centered, minimum height=2cm] (system) at (3.5,1.75) {Biomechanics \\ $\boldsymbol{x}_{t+1}= \boldsymbol{A} \boldsymbol{x}_t + \boldsymbol{z}_{\mathrm{H},t} + \boldsymbol{z}_{\mathrm{A},t}$ };
%$ \boldsymbol{x}_{t+1} = \boldsymbol{f} ( \boldsymbol{x}_t, \boldsymbol{u}_t, t)$
%{Biomechanics \\ $\boldsymbol{x}_{t+1}= \boldsymbol{A} \boldsymbol{x}_t + \boldsymbol{B}_{\mathrm{A}} \boldsymbol{u}_{\mathrm{A},t} $ \\ $ +\boldsymbol{B}_{\mathrm{H}} \boldsymbol{u}_{\mathrm{H},t}  + \boldsymbol{\xi}_t + \sum_i \varepsilon_t^i \boldsymbol{C}_i \boldsymbol{u}_{\mathrm{H},t} $ };


%Box Human
 %inner xsep = 5.5cm, inner ysep=4cm, xshift=-0.5cm
\node[box,  inner xsep = 5.5cm, inner ysep=2.75cm] (boxH) at (-7.5,4.5) {};
 \node [draw=none, anchor=north west, align = right] at (boxH.north west) {Human};
  
  
%Blocks Human
\node[block,  text width=4.5cm] (estimateH) at (-9.5,5.5) {Estimation \\ $\hat{\boldsymbol{x}}_{\mathrm{H},t+1}=\boldsymbol{A} \hat{\boldsymbol{x}}_{\mathrm{H},t}+ \boldsymbol{B}_\mathrm{H} \boldsymbol{u}_{\mathrm{H},t}$ \\ $+\boldsymbol{K}_{\mathrm{H},t}\left(\boldsymbol{y}_{\mathrm{H},t}- \boldsymbol{H}_{\mathrm{H}} \hat{\boldsymbol{x}}_{\mathrm{H},t}\right)$};
%\node[block] (perceptH) at (-7,5.5) {Perception};
\node[block, text width=3cm] (controlH) at (-12.5,3.5) {Control law \\ $\boldsymbol{u}_{\mathrm{H},t} = - \boldsymbol{L}_{\mathrm{H},t} \hat{\boldsymbol{x}}_{\mathrm{H},t} $};

\node[plus] (plusPercept) at (-5,5.5) {};
%Arrows Human
\path[line] (plusPercept) -- (estimateH)node[midway, xshift=0.25cm, yshift=0.25cm](yH){$\boldsymbol{y}_{\mathrm{H},t}$};
\path[line] (estimateH) -- (controlH.north |- estimateH)node[midway, yshift=0.25cm, xshift=-0.25cm](hatxH){$\hat{\boldsymbol{x}}_{\mathrm{H},t}$} -- (controlH);  
\path[line] (controlH) -- (estimateH.south |- controlH)node[midway, yshift=0.25cm, xshift=0cm](uH){$\boldsymbol{u}_{\mathrm{H},t}$} -- (estimateH);  

%Feedback Human
\node (aidSys) at (6.5,1.75) {};
\node[noise] (H_H) at (-3,5.5) {$\boldsymbol{H}_\mathrm{H}$};

\path[line] (system) -- (aidSys.center) -- (H_H.east -| aidSys.center) -- (H_H);%
\path[line] (H_H) -- (plusPercept);
%\path[line] (plusPercept) -- estimateH);

%Perception noise 
\node[noise] (mulPercept) at (-3,6.5) {$\sum_i \epsilon_t^i \boldsymbol{D}_i $};
\node[noiseS] (addPercept) at (-5,6.5) {$\boldsymbol{\omega}_t$};

%Perception arrow in
\node (aidNPIn) at (-0.75,5.5) {};
\path[line] (aidNPIn.center) -- (mulPercept.east -| aidNPIn.center) -- (mulPercept);

%Perception arrow out
\path[line] (mulPercept.west) -- (plusPercept)node[yshift=0cm](plus1){$+$};
\path[line] (addPercept.south) -- (plusPercept);

%Control noise
%helper-nodes
\node[plus] (plusControl) at (-2.5,3.5) {};

%noise
\node[noise] (B_H) at (-5,3.5) {$\boldsymbol{B}_\mathrm{H}$};
\node[noise] (mulControl) at (-5,2.5) {$\sum_i \varepsilon_t^i \boldsymbol{C}_i $};
\node[noiseS] (addControl) at (-2.5,2.5) {$\boldsymbol{\xi}_t$};
%arrow
\path[line] (controlH) -- (B_H);
\path[line] (B_H) -- (plusControl)node[yshift=0cm](plus2){$+$};
\path[line] (mulControl.east) -- (plusControl);
\path[line] (addControl.north) -- (plusControl);

\node (aidNCIn) at (-6.25,3.5) {};
\path[line] (aidNCIn.center) -- (mulControl.west -| aidNCIn.center) -- (mulControl);


%human-->system
\node (aidH) at (0.5,3.5) {};
\node (sysInH) at (1,2.0) {};

\path[line] (plusControl)-- (aidH.center)node[midway, xshift=1.25cm, yshift=0.25cm](zH){$\boldsymbol{z}_{\mathrm{H},t}$} -- (sysInH.west -| aidH.center) -- (sysInH);


%-----------------------


%Box Aut
 %inner xsep = 5.5cm, inner ysep=4cm, xshift=-0.5cm
\node[box,  inner xsep = 5.5cm, inner ysep=2.25cm] (boxA) at (-7.5,-0.75) {};
 \node [draw=none, anchor=north west, align = right] at (boxA.north west) {Automation};
  
%Blocks Aut
\node[block,  text width=4.5cm] (estimateA) at (-8.5,-2) {Estimation \\ $\hat{\boldsymbol{x}}_{\mathrm{A},t+1}=\boldsymbol{A} \hat{\boldsymbol{x}}_{\mathrm{A},t}+ \boldsymbol{B}_\mathrm{A} \boldsymbol{u}_{\mathrm{A},t} $\\$+\boldsymbol{K}_{\mathrm{A},t}\left(\boldsymbol{y}_{\mathrm{A},t}- \boldsymbol{H}_{\mathrm{A}} \hat{\boldsymbol{x}}_{\mathrm{A},t}\right)$};
\node[block] (perceptA) at (-2.5,-2) {Perception $\boldsymbol{H}_\mathrm{A}$};

\node[block, text width=3.5cm] (controlA) at (-12,0) {Control law \\ $\boldsymbol{u}_{\mathrm{A},t} = - \boldsymbol{L}_{\mathrm{A},t} \hat{\boldsymbol{x}}_{\mathrm{A},t} $};

\node[noise] (B_A) at (-2.5,0) {$\boldsymbol{B}_\mathrm{A}$};

\path[line] (perceptA) -- (estimateA)node[midway, yshift=0.25cm](yA){$\boldsymbol{y}_{\mathrm{A},t}$};
\path[line] (estimateA) -- (controlA.north |- estimateA)node[midway, yshift=0.25cm](hatxA){$\hat{\boldsymbol{x}}_{\mathrm{A},t}$} -- (controlA);  
\path[line] (controlA) -- (estimateA.south |- controlA)node[midway, yshift=0.25cm](uA){$\boldsymbol{u}_{\mathrm{A},t}$} -- (estimateA);  


%feedback

\path[line] (system) -- (aidSys.center)node[midway, xshift=0.5cm](yA){$\boldsymbol{x}_t$} -- (perceptA.east -| aidSys.center) -- (perceptA);

%human-->system
\node (aidA) at (0.5,0) {};

\node (sysInA) at (1,1.5) {};

\node (sysInH) at (1,1.0) {};

\path[line] (controlA) -- (B_A);
\path[line] (B_A)-- (aidA.center)node[midway, xshift=1cm, yshift=-0.25cm](zH){$\boldsymbol{z}_{\mathrm{A},t}$} -- (sysInA.west -| aidA.center) -- (sysInA);



%FRAMES

\node[frame,  inner xsep = 1.25cm, inner ysep=1.25cm] (framePercept) at (-3.5,5.8) {};
 \node [draw=none, anchor=south west, align = right] at (framePercept.south west) {Perception};

\node[frame,  inner xsep = 1.25cm, inner ysep=1.25cm] (frameAction) at (-3.5,3.2) {};
 \node [draw=none, anchor=north east, align = right] at (frameAction.north east) {Action};



\end{tikzpicture}

==> 1_tex/img/HRVC_system2.tex <==

 \definecolor{shadecolor}{rgb}{0.92,0.92,0.92}

\tikzstyle{block} = [rectangle, draw, text width=2cm, text centered, minimum height=1.5cm]
 \tikzstyle{box} = [rectangle, draw, fill=shadecolor, text width=9em, text centered, rounded corners, minimum height=4em]
\tikzstyle{noise} = [rectangle, draw, text width=1.5cm, text centered, minimum height=0.8cm]
\tikzstyle{noiseS} = [rectangle, draw, text width=1cm, text centered, minimum height=0.8cm]
\tikzstyle{plus} = [circle, draw, text width=0.1cm, text centered]
 \tikzstyle{frame} = [rectangle, dashed, draw, text width=9em, text centered, minimum height=4em]


\tikzstyle{line} = [draw, -latex']

\usetikzlibrary{arrows}
\begin{tikzpicture}
 
 %system
\node[block, fill=shadecolor, text width=5cm, text centered, minimum height=2cm] (system) at (3.5,1.75) {Biomechanics \\ $\boldsymbol{x}_{t+1}= \boldsymbol{A} \boldsymbol{x}_t + \boldsymbol{z}_{\mathrm{H},t} + \boldsymbol{z}_{\mathrm{A},t}$ };
%$ \boldsymbol{x}_{t+1} = \boldsymbol{f} ( \boldsymbol{x}_t, \boldsymbol{u}_t, t)$
%{Biomechanics \\ $\boldsymbol{x}_{t+1}= \boldsymbol{A} \boldsymbol{x}_t + \boldsymbol{B}_{\mathrm{A}} \boldsymbol{u}_{\mathrm{A},t} $ \\ $ +\boldsymbol{B}_{\mathrm{H}} \boldsymbol{u}_{\mathrm{H},t}  + \boldsymbol{\xi}_t + \sum_i \varepsilon_t^i \boldsymbol{C}_i \boldsymbol{u}_{\mathrm{H},t} $ };


%Box Human
 %inner xsep = 5.5cm, inner ysep=4cm, xshift=-0.5cm
\node[box,  inner xsep = 5.5cm, inner ysep=2.75cm] (boxH) at (-7.5,4.5) {};
 \node [draw=none, anchor=north west, align = right] at (boxH.north west) {Human};
  
  
%Blocks Human
\node[block,  text width=4.5cm] (estimateH) at (-9.5,5.5) {Estimation \\ $\hat{\boldsymbol{x}}_{\mathrm{H},t+1}=\boldsymbol{A} \hat{\boldsymbol{x}}_{\mathrm{H},t}+ \boldsymbol{B}_\mathrm{H} \boldsymbol{u}_{\mathrm{H},t}$ \\ $+\boldsymbol{K}_{\mathrm{H},t}\left(\boldsymbol{y}_{\mathrm{H},t}- \boldsymbol{H}_{\mathrm{H}} \hat{\boldsymbol{x}}_{\mathrm{H},t}\right)$};
%\node[block] (perceptH) at (-7,5.5) {Perception};
\node[block, text width=3cm] (controlH) at (-12.5,3.5) {Control law \\ $\boldsymbol{u}_{\mathrm{H},t} = - \boldsymbol{L}_{\mathrm{H},t} \hat{\boldsymbol{x}}_{\mathrm{H},t} $};

\node[plus] (plusPercept) at (-5,5.5) {};
%Arrows Human
\path[line] (plusPercept) -- (estimateH)node[midway, xshift=0.25cm, yshift=0.25cm](yH){$\boldsymbol{y}_{\mathrm{H},t}$};
\path[line] (estimateH) -- (controlH.north |- estimateH)node[midway, yshift=0.25cm, xshift=-0.25cm](hatxH){$\hat{\boldsymbol{x}}_{\mathrm{H},t}$} -- (controlH);  
\path[line] (controlH) -- (estimateH.south |- controlH)node[midway, yshift=0.25cm, xshift=0cm](uH){$\boldsymbol{u}_{\mathrm{H},t}$} -- (estimateH);  

%Feedback Human
\node (aidSys) at (6.5,1.75) {};
\node[noise] (H_H) at (-3,5.5) {$\boldsymbol{H}_\mathrm{H}$};

\path[line] (system) -- (aidSys.center) -- (H_H.east -| aidSys.center) -- (H_H);%
\path[line] (H_H) -- (plusPercept);
%\path[line] (plusPercept) -- estimateH);

%Perception noise 
\node[noise] (mulPercept) at (-3,6.5) {$\sum_i \epsilon_t^i \boldsymbol{D}_i $};
\node[noiseS] (addPercept) at (-5,6.5) {$\boldsymbol{\omega}_t$};

%Perception arrow in
\node (aidNPIn) at (-0.75,5.5) {};
\path[line] (aidNPIn.center) -- (mulPercept.east -| aidNPIn.center) -- (mulPercept);

%Perception arrow out
\path[line] (mulPercept.west) -- (plusPercept)node[yshift=0cm](plus1){$+$};
\path[line] (addPercept.south) -- (plusPercept);

%Control noise
%helper-nodes
\node[plus] (plusControl) at (-2.5,3.5) {};

%noise
\node[noise] (B_H) at (-5,3.5) {$\boldsymbol{B}_\mathrm{H}$};
\node[noise] (mulControl) at (-5,2.5) {$\sum_i \varepsilon_t^i \boldsymbol{C}_i $};
\node[noiseS] (addControl) at (-2.5,2.5) {$\boldsymbol{\xi}_t$};
%arrow
\path[line] (controlH) -- (B_H);
\path[line] (B_H) -- (plusControl)node[yshift=0cm](plus2){$+$};
\path[line] (mulControl.east) -- (plusControl);
\path[line] (addControl.north) -- (plusControl);

\node (aidNCIn) at (-6.25,3.5) {};
\path[line] (aidNCIn.center) -- (mulControl.west -| aidNCIn.center) -- (mulControl);


%human-->system
\node (aidH) at (0.5,3.5) {};
\node (sysInH) at (1,2.0) {};

\path[line] (plusControl)-- (aidH.center)node[midway, xshift=1.25cm, yshift=0.25cm](zH){$\boldsymbol{z}_{\mathrm{H},t}$} -- (sysInH.west -| aidH.center) -- (sysInH);


%-----------------------


%Box Aut
 %inner xsep = 5.5cm, inner ysep=4cm, xshift=-0.5cm
\node[box,  inner xsep = 5.5cm, inner ysep=2.25cm] (boxA) at (-7.5,-0.75) {};
 \node [draw=none, anchor=north west, align = right] at (boxA.north west) {Automation};
  
%Blocks Aut
\node[block,  text width=4.5cm] (estimateA) at (-8.5,-2) {Estimation \\ $\hat{\boldsymbol{x}}_{\mathrm{A},t+1}=\boldsymbol{A} \hat{\boldsymbol{x}}_{\mathrm{A},t}+ \boldsymbol{B}_\mathrm{A} \boldsymbol{u}_{\mathrm{A},t} $\\$+\boldsymbol{K}_{\mathrm{A},t}\left(\boldsymbol{y}_{\mathrm{A},t}- \boldsymbol{H}_{\mathrm{A}} \hat{\boldsymbol{x}}_{\mathrm{A},t}\right)$};
\node[block] (perceptA) at (-2.5,-2) {Perception $\boldsymbol{H}_\mathrm{A}$};

\node[block, text width=3.5cm] (controlA) at (-12,0) {Control law \\ $\boldsymbol{u}_{\mathrm{A},t} = - \boldsymbol{L}_{\mathrm{A},t} \hat{\boldsymbol{x}}_{\mathrm{A},t} $};

\node[block] (B_A) at (-2.5,0) {Action \\ $\boldsymbol{B}_\mathrm{A}$};

\path[line] (perceptA) -- (estimateA)node[midway, yshift=0.25cm](yA){$\boldsymbol{y}_{\mathrm{A},t}$};
\path[line] (estimateA) -- (controlA.north |- estimateA)node[midway, yshift=0.25cm](hatxA){$\hat{\boldsymbol{x}}_{\mathrm{A},t}$} -- (controlA);  
\path[line] (controlA) -- (estimateA.south |- controlA)node[midway, yshift=0.25cm](uA){$\boldsymbol{u}_{\mathrm{A},t}$} -- (estimateA);  


%feedback

\path[line] (system) -- (aidSys.center)node[midway, xshift=0.5cm](yA){$\boldsymbol{x}_t$} -- (perceptA.east -| aidSys.center) -- (perceptA);

%human-->system
\node (aidA) at (0.5,0) {};

\node (sysInA) at (1,1.5) {};

\node (sysInH) at (1,1.0) {};

\path[line] (controlA) -- (B_A);
\path[line] (B_A)-- (aidA.center)node[midway, xshift=1cm, yshift=-0.25cm](zH){$\boldsymbol{z}_{\mathrm{A},t}$} -- (sysInA.west -| aidA.center) -- (sysInA);



%FRAMES

\node[frame,  inner xsep = 1.25cm, inner ysep=1.25cm] (framePercept) at (-3.5,5.8) {};
 \node [draw=none, anchor=south west, align = right] at (framePercept.south west) {Perception};

\node[frame,  inner xsep = 1.25cm, inner ysep=1.25cm] (frameAction) at (-3.5,3.2) {};
 \node [draw=none, anchor=north east, align = right] at (frameAction.north east) {Action};



\end{tikzpicture}

==> 1_tex/img/HVROC_procedure.tex <==
% \definecolor{r1}{RGB}{0,150,130}
\definecolor{gray1}{RGB}{242,242,242}
\definecolor{gray2}{RGB}{180,180,180}


\usetikzlibrary{arrows}

\tikzstyle{block} = [rectangle, draw, fill=white,
   text width=2cm, text centered, minimum height=4em]
\tikzstyle{box} = [rectangle, draw, text width=24em, text centered,  minimum height=8em] %fill=gray1, rounded corners,
\tikzstyle{line} = [draw, ->] % [draw, -latex']


\begin{tikzpicture}[node distance = 2cm, auto]
    
  	\node [text width = 4.5cm, align=center ] (ident) at (0,10) { $ \boldsymbol{A}, \boldsymbol{B}_\mathrm{H},  \boldsymbol{B}_\mathrm{A},  \boldsymbol{H}_\mathrm{H},  \boldsymbol{H}_\mathrm{A},$ \\ %$\bigA, \bigB_\mathrm{H}, \bigB_\mathrm{A}, \bigH_\mathrm{H}, \bigH_\mathrm{A},$ \\
  	$\boldsymbol{Q}_{\mathrm{H},t}, \boldsymbol{R}_{\mathrm{H}}, 
  	 \boldsymbol{C}_i, \boldsymbol{D}, \boldsymbol{\Sigma}^{\boldsymbol{\omega}}, \boldsymbol{\Sigma}^{\boldsymbol{\xi}},   $}; 
   	\node [block, text width = 6.5cm] (meanHuman) at (0,8) {$\mathrm{E} \{ \boldsymbol{p}_\mathrm{human} \}, \mathrm{cov}(\boldsymbol{p}_\mathrm{human}) $ using~\eqref{eq:E_human},~\eqref{eq:cov_human}};
   	
   	\node [box, inner xsep = 1cm, inner ysep=3cm, anchor=north] (box) at (0,6.5) {};

	%bilevel block
   	\node [block, text width = 9cm] (calcTop) at (0,5) { \begin{align} 
   	\min_{\boldsymbol{q}_\mathrm{A}, \boldsymbol{r}_\mathrm{A}} J_\mathrm{HVROC} \Big( 
   	& \mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \},  \mathrm{E} \{ \boldsymbol{p}_\mathrm{human} \}, \notag \\
   	& \mathrm{cov}(\boldsymbol{p}_\mathrm{HVROC}), \mathrm{cov}(\boldsymbol{p}_\mathrm{human}), \boldsymbol{p}_\mathrm{ref}    \Big)   \notag
   	\end{align}};

	\node [block, text width = 9cm] (calcBot) at (0,1.5) { $
   	\mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \}, 
   	\mathrm{cov}(\boldsymbol{p}_\mathrm{HVROC})  $ by Lemma~\ref{lemma}};

	%arrows bi-level
	\node[xshift=-1cm] (anchorTL) at (calcTop.south) {} ;	
	\node[xshift=-1cm] (anchorBL) at (calcBot.north) {};	
	\path[line] (anchorTL.center) -- (anchorBL.center)node[midway, left](q-r) {$\boldsymbol{q}_{\mathrm{A}}, \boldsymbol{r}_{\mathrm{A}} $};

	\node[xshift=1cm] (anchorTR) at (calcTop.south) {};	
	\node[xshift=1cm] (anchorBR) at (calcBot.north) {};	
	\path[line] (anchorBR.center) -- (anchorTR.center)node[midway, right](q-r) {$ \mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \},  \mathrm{cov}(\boldsymbol{p}_\mathrm{HVROC}) $};
	
	
	%left blocks
	\node [text width = 3cm, align=left] (input) at (-7.5,5) {$\boldsymbol{p}_\mathrm{ref}, \boldsymbol{q}_0, \boldsymbol{r}_0,$ \\
	$\boldsymbol{s} = \begin{bmatrix} s_\mathrm{highMidVar} \\ s_\mathrm{lowMidVar} \\  s_\mathrm{endVar} \\ s_\mathrm{ref} \end{bmatrix}$ };
	
	\path[line] (input) -- (box.west |- input) {};
	
	\node[block] (output) at (0,-1.5) {$\boldsymbol{L}^*_\mathrm{A}$, see~\ref{sec:automation} };
	
	\path[line] (ident) -- (meanHuman);
	\path[line] (meanHuman) -- (box);
	\path[line] (box) -- (output)node[midway](out){$\boldsymbol{q}_{\mathrm{A}}^*, \boldsymbol{r}_{\mathrm{A}}^* $};
	

\end{tikzpicture}


==> 1_tex/img/HVROC_procedure_cov.tex <==
% \definecolor{r1}{RGB}{0,150,130}
\definecolor{gray1}{RGB}{242,242,242}
\definecolor{gray2}{RGB}{180,180,180}


\usetikzlibrary{arrows}

\tikzstyle{block} = [rectangle, draw, fill=white,
   text width=2cm, text centered, minimum height=4em]
\tikzstyle{box} = [rectangle, draw, text width=24em, text centered,  minimum height=8em] %fill=gray1, rounded corners,
\tikzstyle{line} = [draw, ->] % [draw, -latex']


\begin{tikzpicture}[node distance = 2cm, auto]
    
  	\node [text width = 4.5cm, align=center ] (ident) at (0,10) { $ \boldsymbol{A}, \boldsymbol{B}_\mathrm{H},  \boldsymbol{B}_\mathrm{A},  \boldsymbol{H}_\mathrm{H},  \boldsymbol{H}_\mathrm{A},$ \\ %$\bigA, \bigB_\mathrm{H}, \bigB_\mathrm{A}, \bigH_\mathrm{H}, \bigH_\mathrm{A},$ \\
  	$\boldsymbol{Q}_{\mathrm{H},t}, \boldsymbol{R}_{\mathrm{H}}, 
  	 \boldsymbol{C}_i, \boldsymbol{D}, \boldsymbol{\Sigma}^{\boldsymbol{\omega}}, \boldsymbol{\Sigma}^{\boldsymbol{\xi}},   $}; 
   	\node [block, text width = 6.5cm] (meanHuman) at (0,8) {$\mathrm{E} \{ \boldsymbol{p}_\mathrm{human} \}, \mathrm{cov}(\boldsymbol{p}_\mathrm{human}) $ using~\eqref{eq:E_human},~\eqref{eq:cov_human}};
   	
   	\node [box, inner xsep = 1cm, inner ysep=3cm, anchor=north] (box) at (0,6.5) {};

	%bilevel block
   	\node [block, text width = 9cm] (calcTop) at (0,5) { \begin{align}    	
   	\min_{\boldsymbol{q}_\mathrm{A}, \boldsymbol{r}_\mathrm{A}} J_\mathrm{HVROC} \Big( 
   	& \mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \},  \mathrm{E} \{ \boldsymbol{p}_\mathrm{human} \}, \notag \\
   	& \bigOmega_{\mathrm{HVROC}}^{\bigp}, \bigOmega_{\mathrm{human}}^{\bigp}, \boldsymbol{p}_\mathrm{ref}    \Big)   \notag
   	%\min_{\boldsymbol{q}_\mathrm{A}, \boldsymbol{r}_\mathrm{A}} J_\mathrm{HVROC} \Big( 
   	%& \mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \},  \mathrm{E} \{ \boldsymbol{p}_\mathrm{human} \}, \notag \\
   	%& \mathrm{cov}(\boldsymbol{p}_\mathrm{HVROC}), \mathrm{cov}(\boldsymbol{p}_\mathrm{human}), \boldsymbol{p}_\mathrm{ref}    \Big)   \notag
   	\end{align}};

	\node [block, text width = 9cm] (calcBot) at (0,1.5) { $
   	\mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \}, 
   	\bigOmega_{\mathrm{human}}^{\bigp}  $ by Lemma~\ref{lemma}};
   	%\mathrm{cov}(\boldsymbol{p}_\mathrm{HVROC})  $ by Lemma~\ref{lemma}};

	%arrows bi-level
	\node[xshift=-1cm] (anchorTL) at (calcTop.south) {} ;	
	\node[xshift=-1cm] (anchorBL) at (calcBot.north) {};	
	\path[line] (anchorTL.center) -- (anchorBL.center)node[midway, left](q-r) {$\boldsymbol{q}_{\mathrm{A}}, \boldsymbol{r}_{\mathrm{A}} $};

	\node[xshift=1cm] (anchorTR) at (calcTop.south) {};	
	\node[xshift=1cm] (anchorBR) at (calcBot.north) {};	
	\path[line] (anchorBR.center) -- (anchorTR.center)node[midway, right](q-r) {$ \mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \}, \bigOmega_{\mathrm{HVROC}}^{\bigp} $}; %     \mathrm{cov}(\boldsymbol{p}_\mathrm{HVROC}) $};
	
	
	%left blocks
	\node [text width = 3cm, align=left] (input) at (-7.5,5) {$\boldsymbol{p}_\mathrm{ref}, \boldsymbol{q}_0, \boldsymbol{r}_0,$ \\
	$\boldsymbol{s} = \begin{bmatrix} s_\mathrm{highMidVar} \\ s_\mathrm{lowMidVar} \\  s_\mathrm{endVar} \\ s_\mathrm{ref} \end{bmatrix}$ };
	
	\path[line] (input) -- (box.west |- input) {};
	
	\node[block] (output) at (0,-1.5) {$\boldsymbol{L}^*_\mathrm{A}$, see~\ref{sec:automation} };
	
	\path[line] (ident) -- (meanHuman);
	\path[line] (meanHuman) -- (box);
	\path[line] (box) -- (output)node[midway](out){$\boldsymbol{q}_{\mathrm{A}}^*, \boldsymbol{r}_{\mathrm{A}}^* $};
	

\end{tikzpicture}


==> 1_tex/img/HVROC_procedure_cov2.tex <==
% \definecolor{r1}{RGB}{0,150,130}
\definecolor{gray1}{RGB}{242,242,242}
\definecolor{gray2}{RGB}{180,180,180}
 \definecolor{shadecolor}{rgb}{0.92,0.92,0.92}

\usetikzlibrary{arrows}

\tikzstyle{block} = [rectangle, draw, fill=white,
   text width=2cm, text centered, minimum height=3em]
\tikzstyle{box} = [rectangle, fill = shadecolor, draw, text width=24em, text centered,  minimum height=8em] %fill=gray1, rounded corners,
\tikzstyle{line} = [draw, ->] % [draw, -latex']


\begin{tikzpicture}[node distance = 2cm, auto]
    
  	\node [text width = 4.5cm, align=center ] (ident) at (0.5,9.5) { $ \boldsymbol{A}, \boldsymbol{B}_\mathrm{H},  \boldsymbol{B}_\mathrm{A},  \boldsymbol{H}_\mathrm{H},  \boldsymbol{H}_\mathrm{A},$ \\ %$\bigA, \bigB_\mathrm{H}, \bigB_\mathrm{A}, \bigH_\mathrm{H}, \bigH_\mathrm{A},$ \\
  	$\boldsymbol{Q}_{\mathrm{H},t}, \boldsymbol{R}_{\mathrm{H}}, 
  	 \boldsymbol{C}_i, \boldsymbol{D}_i, \boldsymbol{\Sigma}^{\boldsymbol{\omega}}, \boldsymbol{\Sigma}^{\boldsymbol{\xi}}  $}; 
   	\node [block, text width = 2.5cm] (meanHuman) at (0.5,8) { \eqref{eq:E_human}, \eqref{eq:cov_human}};
   	
   	\node [box, inner xsep = 1cm, inner ysep=2.5cm, anchor=north] (box) at (0,6.5) {};

	%bilevel block
   	\node [block, text width = 9cm] (calcTop) at (0,5) { \begin{align}    	
   	\min_{\boldsymbol{q}_\mathrm{A}, \boldsymbol{r}_\mathrm{A}} J_\mathrm{HVROC} \Big( 
   	& \mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \},  \mathrm{E} \{ \boldsymbol{p}_\mathrm{human} \}, \notag \\
   	& \boldsymbol{\Omega}_{\mathrm{HVROC}}^{\boldsymbol{p}}, \boldsymbol{\Omega}_{\mathrm{human}}^{\boldsymbol{p}}, \boldsymbol{p}_\mathrm{ref}    \Big)   \notag
   	%\min_{\boldsymbol{q}_\mathrm{A}, \boldsymbol{r}_\mathrm{A}} J_\mathrm{HVROC} \Big( 
   	%& \mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \},  \mathrm{E} \{ \boldsymbol{p}_\mathrm{human} \}, \notag \\
   	%& \mathrm{cov}(\boldsymbol{p}_\mathrm{HVROC}), \mathrm{cov}(\boldsymbol{p}_\mathrm{human}), \boldsymbol{p}_\mathrm{ref}    \Big)   \notag
   	\end{align}};

	\node [block, text width = 9cm] (calcBot) at (0,2.5) { \eqref{eq:L_A}, \eqref{eq:K_A} $\rightarrow $ Lemma~\ref{lemma}}; %$\boldsymbol{L}_{\mathrm{A},t}$ by
	%$\mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \}, 
   	%\boldsymbol{\Omega}_{\mathrm{HVROC}}^{\boldsymbol{p}}  $  Lemma~\ref{lemma}};
   	%\mathrm{cov}(\boldsymbol{p}_\mathrm{HVROC})  $ by Lemma~\ref{lemma}};

	%arrows bi-level
	\node[xshift=-1cm] (anchorTL) at (calcTop.south) {} ;	
	\node[xshift=-1cm] (anchorBL) at (calcBot.north) {};	
	\path[line] (anchorTL.center) -- (anchorBL.center)node[midway, left](q-r) {$\boldsymbol{q}_{\mathrm{A}}, \boldsymbol{r}_{\mathrm{A}} $};

	\node[xshift=1cm] (anchorTR) at (calcTop.south) {};	
	\node[xshift=1cm] (anchorBR) at (calcBot.north) {};	
	\path[line] (anchorBR.center) -- (anchorTR.center)node[midway,  right](q-r) {$ \mathrm{E} \{ \boldsymbol{p}_\mathrm{HVROC} \}, \boldsymbol{\Omega}_{\mathrm{HVROC}}^{\boldsymbol{p}} $}; %     \mathrm{cov}(\boldsymbol{p}_\mathrm{HVROC}) $};
	
	
	%left blocks
	\node (p_ref) at (-2.5,9.5) {$\boldsymbol{p}_\mathrm{ref}$};
	\node (input) at (-4,7.5) {$\boldsymbol{s}$, $ \boldsymbol{q}_{\mathrm{A},0}, \boldsymbol{r}_{\mathrm{A},0}$
	}; %= \begin{bmatrix} s_\mathrm{highMidVar} \\ s_\mathrm{lowMidVar} \\  s_\mathrm{endVar} \\ s_\mathrm{ref} \end{bmatrix}$ };
	
	\path[line] (input) -- (calcTop.north -| input) {};
	\path[line] (p_ref) -- (box.north -| p_ref) {};
	\path[line]  (meanHuman -| p_ref) -- (meanHuman) {};
	
	\node[block] (output) at (0,0) { \eqref{eq:L_A}, \eqref{eq:K_A} }; % 
	
	\path[line] (ident) -- (meanHuman);
	\path[line] (meanHuman) -- (calcTop.north -| meanHuman)node[midway, yshift=0.25cm,](identHuman){$\mathrm{E} \{ \boldsymbol{p}_\mathrm{human} \}, \boldsymbol{\Omega}_{\mathrm{human}}^{\boldsymbol{p}} $};
	\path[line] (box) -- (output)node[midway](out) {$\boldsymbol{q}_{\mathrm{A}}^*, \boldsymbol{r}_{\mathrm{A}}^* $};
		
	\node (inputHelp) at (5,9.5) {}; 	
	\path[line] (ident) -- (inputHelp.center) -- (inputHelp |- calcBot.east) -- (calcBot.east);
	
	%out
	\node (L_out) at (2.5,0) {$\boldsymbol{L}^*_{\mathrm{A},t}$};
	\path[line] (output) -- (L_out);
	
\end{tikzpicture}

